Leveraging Computational Reuse for Cost- and QoS-Efficient Task Scheduling in Clouds

Cloud-based computing systems could get oversubscribed due to budget constraints of cloud users which causes violation of Quality of Experience(QoE) metrics such as tasks' deadlines. We investigate an approach to achieve robustness against uncertain task arrival and oversubscription through smart reuse of computation while similar tasks are waiting for execution. Our motivation in this study is a cloud-based video streaming engine that processes video streaming tasks in an on-demand manner. We propose a mechanism to identify various types of "mergeable" tasks and determine when it is appropriate to aggregate tasks without affecting QoS of other tasks. Experiment shows that our mechanism can improve robustness of the system and also saves the overall time of using cloud services by more than 14%.

==> Sources/background.tex <==
\section{Background}
\label{sec:background}
\subsection{Video Stream Transcoding}

Video streams, either in form of on-demand streaming or live streaming, usually have to be converted (\ie transcoded) based on the characteristics of clients' devices~\cite{CVSS,vlsc}. Transcoding can encompass operations such as \emph{bit rate adjustment, spatial resolution reduction, temporal resolution (aka frame rate) reduction, and video compression standard (codec) conversion}. Transcoding can be either performed offline or in an online (\ie on-demand) manner for videos that are rarely accessed~\cite{CVSSJournal}.  However, in the case of live video streaming, it is compulsory to transcode videos in an on-demand manner because they are not available for offline processing~\cite{vlsc}.


A video stream, is composed of several sequences. Each sequence itself is composed of multiple \emph{Group Of Pictures} (GOPs) with sequence header at the beginning. Each GOP contains series of frames that begin with $I$ (intra) frame, followed by a number of $P$ (predicted) frames or $B$ (bi-directional predicted) frames. In practice, each GOP is considered as a video streaming task with an individual deadline \cite{jokhio2011analysis,matin_paper}. Deadline violation of any task reduces QoE (Quality of Experience) of  the viewer. 

\subsection{Cloud-based Video Streaming Engine (CVSE)}
While storing multiple versions of the same video to serve different types of display devices is a conventional practice, Cloud-based Video Streaming Engine (CVSE) enables on-demand (\ie lazy) transcoding of video streams~\cite{CVSSJournal}. This is particularly useful for videos that rarely accessed. In fact, it has been proven that video streams have long-tail access pattern~\cite{darwich16} where most of video streams are rarely accessed and only a few percentage of videos are popular (hot)~\cite{miranda}. For instance, in the case of YouTube, it has been reported that only 5\% of videos are frequently accessed and the rest are rarely accessed~\cite{gill2007youtube}. 

In the CVSE architecture, as shown in Figure~\ref{fig:arch}, the Splitter dispatches GOPs of the requested video stream. A GOP transcoding task request (hereafter, called task) includes the operation required along with the corresponding parameters bound to that request. Each arriving task is assigned an individual deadline and a priority by the Admission Control component. Then, the Admission Control sends the task to the batch queue where the task waits to be assigned by the Scheduler to one of multiple Transcoding VMs' queues. Scheduler's batch queue is managed based on a certain scheduling policy, such as FCFS (First-Come-First-Serve), Earliest-Deadline-First (EDF), Max-Urgency-First and Highest-Priority-First~\cite{matin_paper}. Most of scheduling policies are reliant on the Time Estimator component that is aware of the expected execution time of each task type (\ie different transcoding operation) on Transcoding VMs. Such estimation can be obtained based on historic execution time information of different transcoding operations~\cite{CVSS}. 

Once a task is on a local VM queue, its data is fetched to that VM and finally the task gets executed (transcoded). Video Merger component is in charge of merging transcoded GOPs and transfer them to the viewer. Video Merger considers an output window for each video stream to keep track of processed GOPs. The GOPs that are missing (\eg because of a failure) are requested to be resubmitted by the Admission Control component. GOPs of the videos that are getting popular are recognized by the Caching component of CVSE and are stored to enable caching-based computational reuse.

In this paper, we develop our task aggregation mechanism inside Admission Control component of CVSE. For an arriving task, Admission Control can recognize if it is mergeable with the ones exist in the batch queue or local VM queues. Then, the Admission Control decides if the arriving task can be merged with the existing task without causing additional deadline violation for other tasks. It is needless to say that, before these steps, Caching component verifies if the transcoded format of the requested GOP already is already cached or not.
\begin{figure}
\centering
\begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figures/CVSEarch2.pdf}
    \caption{Overview of Cloud-based Video Streaming Engine (CVSE) that is used for on-demand processing of video streams}
    \label{fig:arch}
  \end{minipage}
  \hspace{0.5cm}
\begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figures/FigADC.pdf}
    \caption{Task aggregation mechanism inside Admission Control of CVSE.}
    \label{fig:adc}
  \end{minipage}
\end{figure}


